An empirical comparison of deep-neural-network architectures for next activity prediction using context-enriched process event logs

Researchers have proposed a variety of predictive business process monitoring (PBPM) techniques aiming to predict future process behaviour during the process execution. Especially, techniques for the next activity prediction anticipate great potential in improving operational business processes. To gain more accurate predictions, a plethora of these techniques rely on deep neural networks (DNNs) and consider information about the context, in which the process is running. However, an in-depth comparison of such techniques is missing in the PBPM literature, which prevents researchers and practitioners from selecting the best solution for a given event log. To remedy this problem, we empirically evaluate the predictive quality of three promising DNN architectures, combined with five proven encoding techniques and based on five context-enriched real-life event logs. We provide four findings that can support researchers and practitioners in designing novel PBPM techniques for predicting the next activities.

==> tables/tab_measures.tex <==

\begin{table}[htb]
\centering
\begin{adjustbox}{max width=0.75\textwidth}
\caption{Metrics for measuring predictive quality.}
\label{tab:metrics}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|}
\hline
\textbf{Metrics}   & \textbf{Formula}         \\ \hline
\textit{Accuracy}  
&
$=\frac{1}{n}\sum_{i=1}^{l}s_{i} \frac{tp_{i}+tn_{i}}{tp_{i}+tn_{i}+fp_{i}+fn_{i}}$

\cellcolor[HTML]{FFFFFF}
\\\hline
\textit{Precision} 
&
$=\frac{1}{n}\sum_{i=1}^{l}s_{i} \frac{tp_{i}}{tp_{i}+fp_{i}}$
\\ \hline
\textit{Recall}    
&
$=\frac{1}{n}\sum_{i=1}^{l}s_{i} \frac{tp_{i}}{tp_{i}fn_{i}}$
\\ \hline
\textit{F1-Score}    
&
$=\frac{1}{n}\sum_{i=1}^{l}s_{i} \frac{precision_{i}*recall_{i}}{precision_{i}+recall_{i}}$
\\ \hline
\textit{$AUC_{PR}$} &
$=\frac{1}{n}\sum_{i=1}^{l}s_{i} \int_{0}^{1}precision_{i}d(recall_{i})$
\\ \hline
\end{tabular}%
%\end{adjustbox}
%}
\end{table}

==> tables/tab_overview_findings.tex <==
\begin{table}[ht]
\caption{Overview of research findings.}
\label{tab:findings}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}|l|l|c|c|c|c|@{}}
\toprule
\textit{RF} & \textit{Description}                                           & \textit{Rel. logs} & \textit{\begin{tabular}[c]{@{}c@{}}Control-flow perspective \end{tabular}} & \textit{\begin{tabular}[c]{@{}c@{}}Context perspective\end{tabular}} & \textit{\begin{tabular}[c]{@{}c@{}}Rel. metrics\end{tabular}} \\ \midrule
(1)     
&   
\begin{tabular}[c]{@{}l@{}} The encoding technique has a stronger impact\\ on the predictive quality of deep neural networks\\ than the type of architecture. \end{tabular}
&
all
&

&                                                                         
& 
Accuracy, F1-score                          
\\ \midrule
(2)     
&
\begin{tabular}[c]{@{}l@{}} 
Hash, onehot and binary encoding outperform\\ ordinal and doc2vec encoding regarding the\\ predictive quality of deep neural networks. \end{tabular}
&
bpic2017w, bpic2019, fsp, helpdesk
&

&

&
Accuracy, F1-score
\\ \midrule
%(3)     
%&
%\begin{tabular}[c]{@{}l@{}} 
%Hash encoding has the strongest\\ impact on the predictive quality of\\ deep neural networks \end{tabular}
%&
%bpic2013i, bpic2017w, bpic2019, fsp
%&

%&

%&
%Accuracy, F1-score
%\\ \midrule
(3)     
&
\begin{tabular}[c]{@{}l@{}} 
LSTMs outperforms the other proposed\\ architectures in regards to predictive quality\\ regardless of the encoding technique. \end{tabular}
&
all 
&

&

&
Accuracy, F1-score
\\ \midrule
(4)     
&
\begin{tabular}[c]{@{}l@{}} 
Magnitude of class imbalance and instance to\\ variants ratio impacts overall predictive performance. \end{tabular}
& 
all    
&                          
& 

& 
$AUC_{PR}$
\\ \bottomrule


\end{tabular}%
}
\end{table}
